Constant Delay and Constant Feedback Moving Window Network Coding for Wireless Multicast: Design and Asymptotic Analysis

A major challenge of wireless multicast is to be able to support a large number of users while simultaneously maintaining low delay and low feedback overhead. In this paper, we develop a joint coding and feedback scheme named Moving Window Network Coding with Anonymous Feedback (MWNC-AF) that successfully addresses this challenge. In particular, we show that our scheme simultaneously achieves both a constant decoding delay and a constant feedback overhead, irrespective of the number of receivers $n$, without sacrificing either throughput or reliability. We explicitly characterize the asymptotic decay rate of the tail of the delay distribution, and prove that transmitting a fixed amount of information bits into the MWNC-AF encoder buffer in each time-slot (called "constant data injection process") achieves the fastest decay rate, thus showing how to obtain delay optimality in a large deviation sense. We then investigate the average decoding delay of MWNC-AF, and show that when the traffic load approaches the capacity, the average decoding delay under the constant injection process is at most one half of that under a Bernoulli injection process. In addition, we prove that the per-packet encoding and decoding complexity of MWNC-AF both scale as $O(\log n)$, with the number of receivers $n$. Our simulations further underscore the performance of our scheme through comparisons with other schemes and show that the delay, encoding and decoding complexity are low even for a large number of receivers, demonstrating the efficiency, scalability, and ease of implementability of MWNC-AF.

==> sect21.tex <==
\subsection{Performance Metrics}
Under a given arrival rate of
$\mathbb{E}\{a[t]\}=\lambda~\text{packet}/\text{slot}$, we define several performance
metrics of interest to evaluate a coding scheme,
namely decoding delay, encoding complexity, and
decoding complexity.




%\begin{definition} (Feedback overhead)
%Feedback overhead is measured as the average amount of resource (in
%time or frequency) needed for sending the beacon signal in the feedback channel. % as $t\to \infty$.
%\end{definition}

%For brevity, we take one time of addition and
%multiplication on the finite field as one operation. Let $W[t]$ denote the number of packets participated the encoding operation of $x[t]$ in time-slot $t$. According to \eqref{rand_linear_comb}, $W[t]$ is given by
%\begin{align}
%W[t] &= \left\lfloor A[t]\right\rfloor-Z[t-1].
%\end{align}
%
%
%
%
%
%\begin{definition} (Decoding complexity)
%
%\end{definition}


==> sect31.tex <==
\section{MWNC with Infrequent Anonymous Feedback}\label{sec:IAF}

\begin{figure}[t]
\centering
  \includegraphics[width=3.5in]{figure/Batched_Feedback}
  %\vspace{-0.25cm}
  \caption{Illustration of MWNC with Infrequent Anonymous Feedback.}
  \vspace{-0.5cm}
  \label{fig:batched_feedback}
\end{figure}

We now propose an infrequent anonymous feedback policy that can
further reduce the feedback overhead to $1/B_{AF}$ of the original
MWNC-AF policy. In this policy, anonymous feedback is practiced once
for a frame of $B_{AF}$ packet transmissions, as shown in Figure
\ref{fig:batched_feedback}. If the transmitter cannot detect the
beacon signal, it will remove $B_{AF}$ packets from the encoder
buffer at the end of the frame. Otherwise, no packet will be
removed. If the uplink beacon-based feedback is reliable, we can
ensure that the removed packets are already seen at each receiver,
i.e., the multicast transmissions are reliable. We note that this
policy does not increase the decoding delay, because the decoding
delay is determined by the virtual decoder queue $Q_i[t]$ of each
receiver, and does not depend on the encoder queue $W[t]$. On the
other hand, this policy results in higher encoding and decoding
complexity, because the number of packets participating the encoding
procedure is increased.

If the uplink beacon-based feedback is not reliable, this policy
also provide an easy way to recover the throughput loss due to
feedback error. Specifically, we can postpone the removal time of
the packets by one frame, which provides an extra protection window
of size B_{AF}. In Figure ??, we plot ?? versus B_{AF} .....

Figure

So far, we have seen that the proposed anonymous feedback policy can
be easily generalized to reduce feedback overhead and cope with
feedback error. We further note that this policy can be used for FDD
systems with a minor change of the frame structure: the feedback
time interval can be replaced by a specific feedback frequency
channel. The transmitter broadcast $A[t]$ and $Z[t]$ to the
receivers at the beginning of each frame, and the receivers keep
sending feedback beacon signals during the frame.

